Quantum picturalism for topological cluster-state computing

Topological quantum computing is a way of allowing precise quantum computations to run on noisy and imperfect hardware. One implementation uses surface codes created by forming defects in a highly-entangled cluster state. Such a method of computing is a leading candidate for large-scale quantum computing. However, there has been a lack of sufficiently powerful high-level languages to describe computing in this form without resorting to single-qubit operations, which quickly become prohibitively complex as the system size increases. In this paper we apply the category-theoretic work of Abramsky and Coecke to the topological cluster-state model of quantum computing to give a high-level graphical language that enables direct translation between quantum processes and physical patterns of measurement in a computer - a "compiler language". We give the equivalence between the graphical and topological information flows, and show the applicable rewrite algebra for this computing model. We show that this gives us a native graphical language for the design and analysis of topological quantum algorithms, and finish by discussing the possibilities for automating this process on a large scale.

==> preamble.tex <==
%----------------------------------
% Load in other packages; should really parameterise this
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}

%%% diagrams has nothing to do with red-green pictures
% just ignore this.
\usepackage{diagrams}
\usepackage{latexsym}
\usepackage{stmaryrd}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{url}

\newtheorem{example}{Example}

% \dagg = dagger
\newcommand{\dagg}{^\dagger}
% ddagg = double dagger
\newcommand{\ddagg}{^\ddagger}


\newcommand{\dimm}{\mathrm{dim}}

% aliases
\newcommand{\infinity}{\infty}
\newcommand{\iso}{\cong}
\newcommand{\isomorphism}{\cong}

% ``semantic'' brakets
\newcommand{\denote}[1]{% ---------
\llbracket #1 \rrbracket} 

\newcommand{\sizeof}[1]{% \sizeof{x} == |x|
  \left|#1\right|}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rwd-quantum : helpful macros for writing about quantum theory
%
%
% Inner products bras kets etc 
%
\newcommand{\bra}[1]{%  dirac 'bra'
    \ensuremath{\left\langle #1 \right|}\xspace}

\newcommand{\ket}[1]{%  dirac 'ket'
    \ensuremath{\left|  #1 \right\rangle}\xspace}

\newcommand{\innp}[2]{%  dirac style inner product
    \ensuremath{\langle #1 \mid #2 \rangle}}

\newcommand{\outp}[2]{%  dirac style outer product
    \ensuremath{\left|\left. #1 \rangle\right.\langle\left. #2 \right|\right. }}

\newcommand{\norm}[1]{% define command to get spacing right
        \ensuremath{\left| #1 \right| }}

%% use the proper notation for CZ etc
\newcommand{\CZ}{\ensuremath{\wedge Z}\xspace}
\newcommand{\CX}{\ensuremath{\wedge X}\xspace}
\newcommand{\CNot}{\CX}


%%%% Use this command through out to insert graphics into 
%%%% the text and have them line up properly.
%%%% first param is the desired height of the graphic
%%%% if it is less the 1ex, it might not look good
\newcommand{\inlinegraphic}[2]{
  %% todo -- make this thing calculate the height 
  %% itself based on a global scaling factor
  \dimendef\grafheight=255\dimendef\grafvshift=254
  \grafheight=#1
  \grafvshift=-0.5\grafheight
  \advance\grafvshift by 0.5ex
  \raisebox{\grafvshift}{\includegraphics[height=\grafheight]{images/#2}\xspace}
}

\newcommand{\inline}[1]{
  \raisebox{0.5ex}{\;#1\;}
}

\newcommand{\Odd}{\ensuremath{\mathrm{Odd}}\xspace}

